DMNER: Biomedical Entity Recognition by Detection and Matching

Biomedical named entity recognition (BNER) serves as the foundation for numerous biomedical text mining tasks. Unlike general NER, BNER require a comprehensive grasp of the domain, and incorporating external knowledge beyond training data poses a significant challenge. In this study, we propose a novel BNER framework called DMNER. By leveraging existing entity representation models SAPBERT, we tackle BNER as a two-step process: entity boundary detection and biomedical entity matching. DMNER exhibits applicability across multiple NER scenarios: 1) In supervised NER, we observe that DMNER effectively rectifies the output of baseline NER models, thereby further enhancing performance. 2) In distantly supervised NER, combining MRC and AutoNER as span boundary detectors enables DMNER to achieve satisfactory results. 3) For training NER by merging multiple datasets, we adopt a framework similar to DS-NER but additionally leverage ChatGPT to obtain high-quality phrases in the training. Through extensive experiments conducted on 10 benchmark datasets, we demonstrate the versatility and effectiveness of DMNER.

==> miscs/table_ablation2.tex <==

\begin{table}[htbp] \small
  \centering
  \begin{tabular}{l|P{11mm}|P{9mm}P{9mm}P{9mm}}\toprule
        method            & dict size &  Pre  &  Rec  &  F1    \\ \midrule
        \multicolumn{5}{c}{Unified NER: BIONLP13}  \\ \midrule
        Random            & 4054 & 73.76 & 70.48 & 72.08   \\
        Standard          & 3097 & 72.99 & 92.51 & 81.60   \\ \midrule
        \multicolumn{5}{c}{Supervised NER: NCBI}  \\ \midrule
        Random            & 2250 & 88.52 & 83.28 & 85.82   \\
        Standard          & 1839 & 87.22 & 99.88 & 93.12   \\ \midrule
        \multicolumn{5}{c}{DS NER: BC5CDR}  \\ \midrule
        Random            & 5719 & 90.92 & 76.18 & 82.90   \\
        Standard          & 4074 & 90.68 & 93.93 & 92.28   \\
        \bottomrule
  \end{tabular}
   \caption{The performance of DLNER's BEL module in predicting entity spans varies when using different dictionaries across the three NER tasks.} \label{tab:aba2}
\end{table}
% 在三个NER任务上，DLNER 的 BEL 模块的在使用不同的字典后对实体span预测的表现。

